Language Models are Universal Embedders

In the large language model (LLM) revolution, embedding is a key component of various systems, such as retrieving knowledge or memories for LLMs or building content moderation filters. As such cases span from English to other natural or programming languages, from retrieval to classification and beyond, it is advantageous to build a unified embedding model rather than dedicated ones for each scenario. In this context, the pre-trained multilingual decoder-only large language models, e.g., BLOOM, emerge as a viable backbone option. To assess their potential, we propose straightforward strategies for constructing embedders and introduce a universal evaluation benchmark. Experimental results show that our trained model is proficient at generating good embeddings across languages and tasks, even extending to languages and tasks for which no finetuning/pretraining data is available. We also present detailed analyses and additional evaluations. We hope that this work could encourage the development of more robust open-source universal embedders.

==> tables/c-mteb.tex <==
\begin{table*} %[t!]
\centering
\resizebox{0.88\textwidth}{!}{
\begin{tabular}{l|c|cccccccc}
\toprule[1pt]
 & \bf Avg. &  \bf Class. & \bf Clust. & \bf PairClass. & \bf Rerank. & \bf Retr. & \bf STS \\
\bf \#Datasets ($\rightarrow$) & 35 & 9 & 4 & 2 & 4 & 8 & 8 \\
\midrule
\midrule
stella-large-zh         & 64.54 & 67.62 & 48.65 & 78.72 & 65.98 & 71.02 & 58.3  \\
bge-large-zh-v1.5 \citep{xiao2023c}      & 64.53 & 69.13 & 48.99 & 81.6  & 65.84 & 70.46 & 56.25 \\
stella-base-zh          & 64.16 & 67.77 & 48.7  & 76.09 & 66.95 & 71.07 & 56.54 \\
piccolo-large-zh        & 64.11 & 67.03 & 47.04 & 78.38 & 65.98 & 70.93 & 58.02 \\
piccolo-base-zh         & 63.66 & 66.98 & 47.12 & 76.61 & 66.68 & 71.2  & 55.9  \\
bge-large-zh-noinstruct \citep{xiao2023c} & 63.4  & 68.58 & 50.01 & 76.77 & 64.9  & 70.54 & 53    \\
bge-base-zh-v1.5 \citep{xiao2023c}       & 63.13 & 68.07 & 47.53 & 79.76 & 65.4  & 69.49 & 53.72 \\
multilingual-e5-large \citep{wang2022text} & 58.84 & 67.34 & 48.23 & 69.89 & 56    & 63.66 & 48.44 \\
bge-small-zh-v1.5 \citep{xiao2023c}      & 57.82 & 63.96 & 44.18 & 70.4  & 60.92 & 61.77 & 49.1  \\
m3e-base \citep{m3e}              & 57.79 & 67.52 & 47.68 & 63.99 & 59.34 & 56.91 & 50.47 \\
m3e-large \citep{m3e}              & 57.66 & 68.2  & 48.88 & 64.3  & 59.66 & 54.75 & 50.42 \\
multilingual-e5-base \citep{wang2022text}   & 56.21 & 65.35 & 40.68 & 67.07 & 54.35 & 61.63 & 46.49 \\
multilingual-e5-small \citep{wang2022text}  & 56.11 & 65.85 & 45.26 & 66.45 & 53.86 & 59.95 & 45.27 \\
text-embedding-ada-002  & 53.73 & 64.31 & 45.68 & 69.56 & 54.28 & 52    & 43.35 \\
\midrule
sgpt-bloom-7b1-msmarco \citep{Scao2022BLOOMA1}  & 41.25 & 64.33 & 28.42 & 57.64 & 47.37 & 33.86 & 30.29 \\
\midrule
\modelname-bloom-560m & 51.34 & 65.63 & 42.42 & 72.38 & 53.63 & 46.16 & 42.80 \\
\modelname-bloom-1b1  & 55.72 & 68.01 & 42.42 & 74.96 & 56.28 & 57.97 & 44.39 \\
\modelname-bloom-3b   & 57.29 & 69.67 & 43.24 & 76.59 & 57.68 & 59.77 & 46.15 \\
\modelname-bloom-7b1  & 58.57 & 70.36 & 42.33 & 78.65 & 59.12 & 62.87 & 46.78 \\
\bottomrule[1pt]
\end{tabular}}
\caption{
Results on MTEB Chinese subset (C-MTEB \citep{xiao2023c}). We include the scores of top-performing models from the online leaderboard (retrieved on October 8th, 2023). The results of sgpt-bloom-7b1-msmarco are evaluated with the oneline model checkpoint.
% In contrast to the baseline \texttt{sgpt-bloom-7b1-msmarco}, \modelname-bloom-7b1 achieve significant improvements on all tasks except summarization (\textbf{Summ.}).
% Full results on each dataset refer to Table \ref{tab:mteb-en-full}.
}
\label{tab:mteb-zh-results}
\end{table*}


==> tables/main.tex <==
\begin{table*}[tbp]
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{cc|rrrrrrrrrrrrrrr|rrr}
\toprule
Language    &  Eval $\rightarrow$  & \multicolumn{3}{c}{English} & \multicolumn{3}{c}{Chinese} & \multicolumn{3}{c}{Arabic} & \multicolumn{3}{c}{Indonesian} & \multicolumn{3}{c}{Java} & \multicolumn{3}{|c}{Average} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} \cmidrule(lr){15-17} \cmidrule(lr){18-20}
& Train $\downarrow$ & asym     & sym     & all    & asym     & sym     & all    & asym      & sym      & all     & asym     & sym    & all    & asym      & sym      & all     & asym    & sym    & all   \\
\midrule
\multirow{3}{*}{English}
& asym   & \bf 39.35 & 72.86 & 56.10 & 31.99 & 69.61 & 50.80 & 36.93 & 61.64 & 49.28 & 20.06 & 63.59 & 41.82 & 46.86 & 58.59 & 52.73 & 35.04 & 65.26 & 50.15 \\
& sym   & 5.38 & \bf 77.04 & 41.21 & 4.31 & 73.76 & 39.04 & 2.53 & 64.14 & 33.34 & 3.55 & 69.07 & 36.31 & 38.63 & 58.38 & 48.50 & 10.88 & 68.48 & 39.68 \\
& all  & 38.60 & 75.95 & \bf 57.27 & 30.88 & 72.75 & 51.81 & 34.87 & 64.39 & 49.63 & 21.14 & 68.45 & 44.79 & 49.39 & 59.05 & 54.22 & 34.98 & 68.12 & 51.55 \\
\midrule
\multirow{3}{*}{Chinese}
& asym  & \uline{34.02} & 73.19 & 53.60 & \bf 36.03 & 70.59 & 53.31 & 34.07 & 62.62 & 48.35 & 17.73 & 64.64 & 41.18 & 46.61 & 59.09 & 52.85 & 33.69 & 66.03 & 49.86 \\
& sym   & 5.00 & \uline{76.36} & 40.68 & 5.88 & \bf 74.66 & 40.27 & 3.18 & 63.91 & 33.55 & 2.37 & 69.71 & 36.04 & 37.00 & 58.03 & 47.52 & 10.69 & 68.53 & 39.61 \\
& all   & 33.16 & 75.39 & \uline{54.27} & 35.95 & 73.46 & \bf 54.70 & 34.86 & 64.78 & 49.82 & 19.30 & 67.94 & 43.62 & 47.13 & 59.19 & 53.16 & 34.08 & 68.15 & 51.11 \\
\midrule
\multirow{3}{*}{Arabic}
& asym  & \uline{32.25} & 72.99 & 52.62 & 8.33 & 64.41 & 36.37 & \bf 42.18 & 62.49 & 52.34 & 17.79 & 61.70 & 39.74 & 41.46 & 55.64 & 48.55 & 28.40 & 63.45 & 45.92 \\
& sym   & 5.63 & 76.47 & 41.05 & 4.45 & 73.87 & 39.16 & 7.72 & \bf 67.14 & 37.43 & 5.66 & 72.14 & 38.90 & 35.87 & 55.29 & 45.58 & 11.87 & 68.98 & 40.42 \\
& all   & 31.69 & 75.83 & 53.76 & 6.41 & 71.54 & 38.98 & 40.96 & 66.85 & \bf 53.91 & 21.96 & 68.18 & 45.07 & 44.92 & 57.57 & 51.24 & 29.19 & 67.99 & 48.59 \\
\midrule
\multirow{3}{*}{Indonesian}
& asym  & 35.89 & 73.12 & 54.50 & 34.10 & 70.22 & 52.16 & 39.00 & 62.57 & 50.79 & \bf 35.73 & 70.00 & 52.87 & 47.09 & 58.81 & 52.95 & \bf 38.36 & 66.94 & 52.65 \\
& sym   & 6.54 & 75.88 & 41.21 & 5.33 & 74.01 & 39.67 & 3.64 & 65.69 & 34.67 & 5.97 & \bf 73.66 & 39.81 & 34.80 & 57.40 & 46.10 & 11.25 & \bf 69.33 & 40.29 \\
& all   & 35.48 & 75.38 & 55.43 & 32.09 & 72.93 & 52.51 & 37.55 & 65.25 & 51.40 & 34.85 & 73.13 & \bf 53.99 & 47.61 & 58.01 & 52.81 & 37.52 & 68.94 & \bf 53.23 \\
\midrule
\multirow{3}{*}{Java}
& asym  & 14.55 & 69.89 & 42.22 & 17.79 & 70.00 & 43.89 & 11.37 & 59.26 & 35.32 & 7.73 & 63.94 & 35.83 & \bf 51.24 & 55.49 & 53.36 & 20.53 & 63.71 & 42.12\\
& sym   & 0.00 & 31.96 & 15.98 & 0.00 & 35.12 & 17.56 & 0.00 & 25.02 & 12.51 & 0.02 & 35.50 & 17.76 & 1.00 & 73.36 & 37.18 & 0.20 & 40.20 & 20.20\\
& all   & 12.77 & 69.98 & 41.38 & 13.75 & 69.78 & 41.76 & 9.18 & 58.74 & 33.96 & 6.93 & 64.11 & 35.52 & 48.70 & \bf 75.85 & \bf 62.28 & 18.27 & 67.69 & 42.98 \\
\bottomrule
\end{tabular}}
\caption{
Main Results on bloom 560m. The socre of the \texttt{asym} (or \texttt{sym}) is the macro average of a in-domain test and a out-of-domain test. All tests are listed in \S\ref{sec:exp-design}. The score of the \texttt{all} is the macro average of \texttt{asym} and \texttt{sym}.
% For natural languages, the evaluation benchmarks of \texttt{asym} include mMarco and MIRACL, that of the \texttt{sym} comprise STS17 (from SNLI, we translate zh id), STS-B (deepl translated) and MassiveIntentClassification.
% For Java, the \texttt{asym} are CodeSearchNet and xCodeEval/nl-to-code-search, while the \texttt{sym} are BigCloneBench and GoogleCodeJam.
% 都是 one in-domain + one out-of-domain
}
% WebQueryTest 是分类
\label{tab:main}
\end{table*}

==> tables/massive.tex <==
\begin{table*}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccccccc}
\toprule[1pt]
\bf Model                                    & \bf ar & \bf bn & \bf en & \bf es & \bf fr & \bf hi & \bf id & \bf kn & \bf ml & \bf pt & \bf sw & \bf ta & \bf te & \bf ur & \bf vi \\
\midrule
% random\_embedding                           & 26.24 & 28.74 & 48.85 & 47.64 & 44.56 & 23.21 & 48.28 & 3.95  & 2.81  & 48.66 & 48.14 & 17.38 & 2.83  & 28.24 & 46.77 \\
LASER2 \citep{heffernan-etal-2022-bitext}   & 37.16 & 42.51 & 47.91 & 45.44 & 46.13 & 40.2  & 45.81 & 4.32  & 41.33 & 48.55 & 31.89 & 29.63 & 36.03 & 26.11 & 44.33 \\
LaBSE \citep{feng-etal-2022-language}       & 50.86 & 58.22 & 61.46 & 58.32 & 60.47 & 59.4  & 61.12 & 56.24 & 57.91 & 60.16 & 51.62 & 55.04 & 58.32 & 56.7  & 56.67 \\
paraphrase-multilingual-mpnet-base-v2       & 51.43 & 48.79 & 69.32 & 64.43 & 64.82 & 62.77 & 65.43 & 50.63 & 54.34 & 64.89 & 31.95 & 50.17 & 52.82 & 56.37 & 59.68 \\
paraphrase-multilingual-MiniLM-L12-v2       & 45.14 & 35.34 & 66.84 & 59.66 & 60.25 & 58.37 & 59.85 & 40.98 & 42.41 & 61.27 & 29.57 & 36.77 & 40.72 & 52.8  & 56.61 \\
sgpt-bloom-7b1-msmarco                      & 59.25 & 61.59 & 69.67 & 66.35 & 66.95 & 63.54 & 64.06 & 53.54 & 58.27 & 66.69 & 49.81 & 56.4  & 54.71 & 56.75 & 64.53 \\
% SGPT-125M-weightedmean-msmarco-specb-bitfit & 30.13 & 29.17 & 61.41 & 42.68 & 43.44 & 27.04 & 43.97 & 23.48 & 24.91 & 45.21 & 41.12 & 24.6  & 25.04 & 25.93 & 38.8  \\
% SGPT-125M-weightedmean-nli-bitfit           & 29.64 & 26.55 & 58.08 & 41.18 & 43.67 & 28.04 & 41.16 & 17.83 & 17.89 & 44.54 & 38.33 & 19.03 & 19.38 & 27.83 & 38.71 \\
% all-MiniLM-L12-v2                           & 20.94 & 13.67 & 67.15 & 40.91 & 44.82 & 17.98 & 39.66 & 3.08  & 2.85  & 45.12 & 35.28 & 13.1  & 2.56  & 16.18 & 37.38 \\
multilingual-e5-base                          & 57.46 & 61.13 & \bf 72.11 & \bf 68.4  & 67.95 & 64.95 & \bf 66.64 & \bf 59.19 & \bf 63.09 & \bf 68.98 & \bf 56    & 58.71 & \bf 59.72 & \bf 61.52 & \bf 66.17 \\
% gtr-t5-xl                                   & 4.64  & 2.84  & 70.23 & 56.72 & 57.67 & 3.24  & 46.54 & 3.17  & 3.18  & 57.03 & 35.85 & 2.32  & 2.2   & 3     & 30.01 \\
% sentence-t5-xl                              & 4.18  & 2.6   & 72.09 & 57.97 & 60.99 & 3.02  & 41.53 & 2.79  & 2.98  & 57.95 & 30.6  & 1.79  & 2.26  & 2.7   & 21.47 \\
% gtr-t5-large                                & 4.87  & 2.52  & 70.06 & 53.3  & 54.83 & 2.88  & 40.11 & 2.44  & 2.67  & 52.27 & 35.97 & 1.52  & 2.57  & 2.57  & 25.23 \\
% sentence-t5-large                           & 4.7   & 2.77  & 71.78 & 54.1  & 57.01 & 2.97  & 34.55 & 2.41  & 2.95  & 51.96 & 31.9  & 1.91  & 2.54  & 2.62  & 22.81 \\
% allenai-specter                             & 10.04 & 3.02  & 51.73 & 35.6  & 38.41 & 3.43  & 40.02 & 3.54  & 2.88  & 43.05 & 34.81 & 3.11  & 2.53  & 9.61  & 37.07 \\
% sentence-t5-base                            & 4.53  & 2.58  & 69.74 & 45.32 & 51.13 & 2.68  & 35.5  & 2.59  & 2.55  & 43.35 & 32.14 & 1.41  & 2.5   & 2.99  & 22.62
\midrule
\modelname-bloom-560m  & 53.38 & 56.74 & 66.09 & 61.17 & 62.61 & 59.46 & 59.14 & 47.97 & 53.69 & 61.74 & 45.55 & 51.24 & 47.43 & 51.85 & 58.72 \\
\modelname-bloom-1b1   & 57.08 & 61.37 & 67.93 & 63.81 & 65.34 & 62.89 & 62.11 & 52.33 & 57.75 & 64.74 & 46.46 & 55.46 & 51.41 & 54.72 & 62.01 \\
\modelname-bloom-3b    & 59.58 & 63.86 & 70.41 & 67.34 & 67.69 & 66.18 & 63.77 & 55.98 & 62.45 & 67.59 & 47.45 & 58.64 & 57.92 & 58.95 & 64.06 \\
\modelname-bloom-7b1   & \bf 60.56 & \bf 64.18 & 72.06 & 67.60 & \bf 68.42 & \bf 66.43 & 65.10 & 56.89 & 62.97 & 68.18 & 48.72 & \bf 59.79 & 58.40 & 59.92 & 65.40 \\
\bottomrule[1pt]
\end{tabular}
}\caption{
Accuracy scores on the MASSIVE \citep{fitzgerald2022massive} test (\ie MassiveIntentClassification in MTEB) of 15 languages covered by BLOOM pre-training.
Scores of competitors are retrieved on June 20th, 2023.
}\label{tab:massive-results}
\end{table*}


==> tables/miracl.tex <==
\begin{table*}[t!]
\centering
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Language}} & \multirow{2}{*}{\textbf{ISO}}  & \multicolumn{5}{c}{\textbf{nDCG@10}} & \multicolumn{5}{c}{\textbf{Recall@100}} \\
& & \textbf{BM25} & \textbf{mDPR} & \textbf{Cohere} & \textbf{bloom-560m} & \textbf{bloom-1b1} & \textbf{bloom-3b} & \textbf{BM25} & \textbf{mDPR} & \textbf{bloom-560m} & \textbf{bloom-1b1} & \textbf{bloom-3b} \\
\cmidrule(lr){1-2} \cmidrule(lr){3-8} \cmidrule(lr){9-13} 
Arabic & Ar & 0.481 & 0.499 & \textbf{0.617} & 0.510 & 0.593 & 0.527 & \textbf{0.889} & 0.841 & 0.832 & 0.884 & 0.818 \\
Bengali & Bn & 0.508 & 0.443 & 0.594 & 0.451 & 0.547 & \textbf{0.614} & 0.909 & 0.819 & 0.794 & 0.897 & \textbf{0.937} \\
English & En & 0.351 & 0.394 & - & 0.405 & 0.443 & \textbf{0.477} & 0.819 & 0.768 & 0.745 & 0.783 & \textbf{0.832} \\
Spanish & Es & 0.319 & 0.478 & \textbf{0.641} & 0.443 & 0.470 & 0.503 & 0.702 & 0.864 & 0.737 & 0.798 & \textbf{0.845} \\
Persian & Fa & 0.333 & 0.480 & \textbf{0.594} & 0.103 & 0.134 & 0.122 & 0.731 & \textbf{0.898} & 0.327 & 0.371 & 0.354  \\
Finnish & Fi & 0.551 & 0.472 &  \textbf{0.672} & 0.129 & 0.191 & 0.192 & \textbf{0.891} & 0.788 & 0.297 & 0.437 & 0.439 \\
French & Fr & 0.183 & 0.435 & 0.523 & 0.427 & 0.453 & \textbf{0.524} & 0.653 & \textbf{0.915} & 0.838 & 0.871 & 0.898 \\
Hindi & Hi & 0.458 & 0.383 & \textbf{0.616} & 0.387 & 0.422 & 0.494 & \textbf{0.868} & 0.776 & 0.788 & 0.811 & 0.856\\
Indonesian & Id & \textbf{0.449} & 0.272 & 0.443 & 0.386 & 0.407 & 0.405 & \textbf{0.904} & 0.573 & 0.698 & 0.712 & 0.717 \\
Japanese & Ja & 0.369 & 0.439 & \textbf{0.576} & 0.239 & 0.274 & 0.299 & \textbf{0.805} & 0.825 & 0.587 & 0.604 & 0.650 \\
Korean & Ko & 0.419 & 0.419 & \textbf{0.609} & 0.059 & 0.083 & 0.103 & \textbf{0.783} & 0.737 & 0.146 & 0.199 & 0.237 \\
Russian & Ru & 0.334 & 0.407 & \textbf{0.532} & 0.103 & 0.132 & 0.268 & 0.661 & \textbf{0.797} & 0.284 & 0.342 & 0.520 \\
Swahili & Sw & 0.383 & 0.299 & \textbf{0.446} & 0.259 & 0.377 & 0.415 & 0.701 & 0.616 & 0.528 & 0.697 & \textbf{0.718} \\
Telugu & Te & 0.494 & 0.356 &  \textbf{0.602} & 0.189 & 0.373 & 0.467 & 0.831 & 0.762 & 0.456 & 0.708 & \textbf{0.848} \\
Thai & Th & 0.484 & 0.358 & \textbf{0.599} & 0.004 & 0.008 & 0.012 & \textbf{0.887} & 0.678 & 0.013 & 0.029 & 0.048\\
Chinese & Zh & 0.180 & 0.512 & \textbf{0.526} & 0.363 & 0.456 & 0.510 & 0.560 & \textbf{0.944} & 0.737 & 0.853 & 0.904 \\
\cmidrule(lr){1-2} \cmidrule(lr){3-8} \cmidrule(lr){9-13} 
% Average & & 0.393 & 0.415 & 0.278 & 0.335 & 0.370 & 0.787 & 0.788 & 0.550 & 0.624 & 0.663 \\
Best on & & 1 & 0 & 12 & 0 & 0 & 3 & 7 & 4 & 0 & 0 & 5 \\
\bottomrule
\end{tabular}
}
\caption{Results on the MIRACL \citep{zhang2022making}, including scores of BM25 and mDPR in their experiments. The scores of Cohere API are taken from \citep{kamalloo2023evaluating} (English result is not presented in the paper).}
\label{tab:mircal}
\end{table*}


==> tables/mteb-en-full.tex <==
\begin{table*}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|lllllllll|cccc}
\toprule[1pt]
 & e5-  & instructor & instructor & e5- & e5- & text-embed & e5- & sgpt-bloom- & SGPT- & \multicolumn{4}{c}{en-all-bloom} \\
Dataset                                & large-v2 & -xl & -large & base-v2 & large & -ding-ada-002 & base & 7b1-msmarco & 5.8B-msmarco & 560m & 1b1 & 3b & 7b1 \\
\midrule \midrule
AmazonCounterfactualClassification     & 79.22 & 85.09 & 88.13 & 77.78 & 77.69 & 75.94 & 79.72 & 68.06 & 69.22    & 72.34 & 69.94 & 78.90 & 73.12 \\
AmazonPolarityClassification           & 93.75 & 86.54 & 91.53 & 92.81 & 90.05 & 86.72 & 87.96 & 68.97 & 71.26    & 83.81 & 87.19 & 87.98 & 88.89 \\
AmazonReviewsClassification            & 48.61 & 42.96 & 47.86 & 46.71 & 43.02 & 44.78 & 42.65 & 33.86 & 39.19    & 38.96 & 41.08 & 42.58 & 43.20 \\
Banking77Classification                & 84.55 & 82.66 & 78.51 & 83.53 & 84.14 & 80.66 & 83.33 & 84.33 & 84.49    & 80.97 & 82.89 & 84.16 & 85.36 \\
EmotionClassification                  & 49.45 & 53.24 & 52.73 & 46.95 & 48.05 & 48.74 & 49.44 & 44.87 & 49.66    & 44.77 & 46.84 & 47.88 & 48.76 \\
ImdbClassification                     & 91.69 & 79.79 & 88.32 & 86.15 & 82.11 & 77.98 & 75.96 & 61.77 & 66.64    & 72.21 & 74.45 & 77.70 & 78.46 \\
MTOPDomainClassification               & 94.62 & 95.07 & 93.89 & 93.69 & 93.86 & 92.13 & 93.21 & 93.68 & 93.47    & 89.94 & 92.19 & 92.34 & 93.43 \\
MTOPIntentClassification               & 77.14 & 72.26 & 67.98 & 75.31 & 76.4  & 64.68 & 74.77 & 71.34 & 72.42    & 66.57 & 70.31 & 70.63 & 71.73 \\
MassiveIntentClassification            & 73.84 & 71.48 & 68.9  & 73.04 & 73.22 & 70.15 & 72.25 & 69.67 & 70.39    & 66.10 & 68.01 & 70.39 & 72.04 \\
MassiveScenarioClassification          & 78.11 & 76.47 & 73.35 & 77.65 & 77.39 & 75.33 & 76.76 & 75.34 & 76.28    & 73.25 & 75.70 & 77.19 & 76.86 \\
ToxicConversationsClassification       & 70.9  & 70.33 & 71.05 & 72.11 & 70.56 & 72.29 & 74.12 & 66.55 & 67.71    & 67.96 & 72.01 & 72.13 & 71.58 \\
TweetSentimentExtractionClassification & 60.94 & 61.58 & 64.13 & 60.39 & 61.21 & 61.81 & 61.38 & 55.85 & 56.85    & 59.60 & 61.51 & 61.04 & 62.14 \\
\midrule
ArxivClusteringP2P                     & 45.55 & 42.45 & 43.16 & 46.1  & 46.19 & 45.01 & 44.57 & 44.59 & 45.59    & 40.27 & 44.52 & 45.37 & 45.66 \\
ArxivClusteringS2S                     & 41.02 & 32.21 & 32.56 & 39.67 & 41.38 & 36.85 & 40.48 & 38.03 & 38.86    & 32.00 & 34.45 & 36.52 & 38.42 \\
BiorxivClusteringP2P                   & 37.36 & 37.37 & 37.62 & 37.5  & 37.6  & 36.66 & 36.19 & 36.03 & 36.55    & 33.27 & 35.25 & 36.52 & 35.54 \\
BiorxivClusteringS2S                   & 34.85 & 30.55 & 31.33 & 32.72 & 35.09 & 34.21 & 32.72 & 32.48 & 33.7     & 28.65 & 30.71 & 31.98 & 32.19 \\
MedrxivClusteringP2P                   & 31.82 & 33.19 & 34.22 & 31.46 & 32.26 & 32.6  & 31.53 & 31.05 & 31.51    & 27.85 & 29.43 & 31.71 & 30.95 \\
MedrxivClusteringS2S                   & 30.38 & 30.79 & 32    & 28.99 & 29.66 & 30.8  & 28.29 & 29.26 & 28.76    & 27.71 & 28.87 & 28.80 & 28.87 \\
RedditClustering                       & 55.83 & 63.49 & 63.65 & 56.16 & 50.69 & 61.42 & 48.18 & 35.53 & 40.45    & 41.34 & 44.52 & 49.71 & 47.90 \\
RedditClusteringP2P                    & 63.38 & 65.13 & 64.63 & 63.43 & 61.37 & 64.13 & 62.19 & 54.52 & 55.75    & 51.20 & 53.61 & 55.07 & 55.95 \\
StackExchangeClustering                & 65.92 & 68.44 & 68.78 & 65.15 & 64.96 & 72.22 & 63.91 & 55.13 & 59.21    & 54.51 & 57.11 & 59.42 & 60.27 \\
StackExchangeClusteringP2P             & 33.67 & 35.17 & 36.15 & 32.5  & 33.6  & 38.49 & 32.56 & 34.31 & 33.95    & 31.12 & 31.91 & 31.70 & 32.34 \\
TwentyNewsgroupsClustering             & 49.6  & 53.38 & 54.13 & 48.16 & 43.81 & 52.56 & 42.58 & 37.28 & 39.46    & 37.88 & 39.80 & 41.29 & 40.81 \\
\midrule
SprintDuplicateQuestions               & 94.92 & 94.94 & 93.07 & 94.58 & 95.42 & 92.17 & 94.88 & 94.93 & 93.84    & 92.09 & 94.58 & 95.36 & 95.62 \\
TwitterSemEval2015                     & 76.92 & 77.99 & 77.42 & 75.97 & 76.1  & 75.28 & 74.4  & 65.31 & 66.87    & 65.96 & 69.14 & 70.64 & 73.81 \\
TwitterURLCorpus                       & 86.25 & 86.93 & 87.18 & 86.63 & 86.31 & 87.22 & 85.98 & 85.46 & 85.29    & 85.11 & 85.62 & 86.18 & 86.78 \\
\midrule
AskUbuntuDupQuestions                  & 59.62 & 65.35 & 64.3  & 58.98 & 60.07 & 62.05 & 59.66 & 59.97 & 61.63    & 57.38 & 59.50 & 59.92 & 61.60 \\
MindSmallReranking                     & 31.83 & 31.81 & 31.68 & 31.29 & 30.78 & 31.45 & 30.07 & 31.79 & 32.29    & 30.52 & 30.51 & 30.97 & 31.22 \\
SciDocsRR                              & 84.31 & 79.49 & 82    & 83.02 & 83.94 & 81.22 & 82.9  & 79.77 & 80.79    & 75.13 & 78.11 & 78.62 & 80.27 \\
StackOverflowDupQuestions              & 50.68 & 52.52 & 52.17 & 50.34 & 51.33 & 50.54 & 50.15 & 51.07 & 51.53    & 47.38 & 49.00 & 50.07 & 50.55 \\
\midrule
ArguAna                                & 46.42 & 55.65 & 57.05 & 44.49 & 49.35 & 57.44 & 51.41 & 47.28 & 51.38    & 44.54 & 46.67 & 48.33 & 52.21 \\
CQADupstackRetrieval                   & 37.89 & 43.09 & 43.82 & 38.54 & 39.44 & 41.69 & 38.92 & 39.62 & 39.4     & 31.43 & 34.30 & 37.82 & 39.29 \\
ClimateFEVER                           & 22.21 & 26.54 & 27.74 & 26.56 & 22.4  & 21.64 & 15.38 & 29.39 & 30.46    & 21.02 & 25.56 & 23.36 & 26.79 \\
DBPedia                                & 44.02 & 40.24 & 36.68 & 42.23 & 42.39 & 39.39 & 41.02 & 39.03 & 39.87    & 28.22 & 32.61 & 34.54 & 37.62 \\
FEVER                                  & 82.83 & 70.03 & 72.69 & 84.99 & 65.03 & 74.99 & 58.24 & 73.97 & 78.24    & 61.10 & 67.22 & 71.96 & 73.98 \\
FiQA2018                               & 41.14 & 46.96 & 45.45 & 39.88 & 38.56 & 44.41 & 36.37 & 35.84 & 37.2     & 24.49 & 31.29 & 35.12 & 36.70 \\
HotpotQA                               & 73.13 & 55.88 & 55.18 & 69.15 & 63.33 & 60.9  & 62.21 & 57.26 & 59.26    & 46.05 & 51.67 & 55.12 & 56.66 \\
MSMARCO                                & 43.46 & 41.61 & 39.65 & 41.77 & 44.05 & 40.91 & 43.14 & 41.12 & 39.91    & 34.18 & 38.27 & 40.25 & 42.02 \\
NFCorpus                               & 37.13 & 36    & 34.09 & 35.39 & 36.07 & 36.97 & 36.59 & 35.78 & 36.21    & 27.34 & 30.70 & 33.66 & 36.02 \\
NQ                                     & 63.44 & 57.24 & 50.1  & 58.22 & 62.86 & 51.58 & 59.97 & 53.15 & 52.41    & 40.05 & 46.16 & 50.62 & 53.31 \\
QuoraRetrieval                         & 86.84 & 88.85 & 88.44 & 86.56 & 88.18 & 87.6  & 87.92 & 74.71 & 84.58    & 86.04 & 87.01 & 88.01 & 88.28 \\
SCIDOCS                                & 20.51 & 17.36 & 18.55 & 18.69 & 20.12 & 18.36 & 18.99 & 18.62 & 19.87    & 15.31 & 17.24 & 18.50 & 18.94 \\
SciFact                                & 72.24 & 64.56 & 64.43 & 71.94 & 72.58 & 72.75 & 73.08 & 72.11 & 74.7     & 61.74 & 65.42 & 69.43 & 69.29 \\
TRECCOVID                              & 66.54 & 71.4  & 58.06 & 69.6  & 78.32 & 68.47 & 79.64 & 81.37 & 84.88    & 72.99 & 80.03 & 83.21 & 83.82 \\
Touche2020                             & 20.67 & 23.44 & 21.56 & 26.4  & 27.21 & 21.61 & 28.31 & 23.98 & 25.43    & 23.35 & 24.92 & 25.17 & 25.19 \\
\midrule
BIOSSES                                & 83.6  & 84.15 & 84.39 & 81.4  & 84.73 & 86.35 & 85.1  & 85.31 & 86.25    & 84.44 & 84.65 & 84.82 & 85.52 \\
SICK-R                                 & 79.28 & 81.7  & 81.27 & 78.3  & 80.49 & 80.6  & 79.66 & 69.82 & 69.63    & 78.53 & 79.92 & 80.85 & 81.41 \\
STS12                                  & 76.95 & 75.32 & 76.28 & 75.79 & 75.93 & 69.8  & 74.22 & 69.66 & 67.5     & 74.07 & 75.80 & 76.10 & 77.47 \\
STS13                                  & 84.12 & 87.44 & 88.18 & 83.58 & 85.22 & 83.27 & 83.31 & 79.67 & 79.16    & 81.81 & 83.62 & 85.49 & 86.38 \\
STS14                                  & 80.46 & 81.87 & 81.92 & 79.95 & 80.54 & 76.09 & 78.52 & 74.61 & 74.46    & 77.05 & 78.73 & 80.44 & 81.17 \\
STS15                                  & 89.76 & 88.94 & 89.01 & 88.82 & 88.81 & 86.12 & 88.35 & 83.81 & 84.47    & 84.61 & 86.41 & 87.75 & 88.23 \\
STS16                                  & 85.47 & 85.38 & 85.49 & 84.46 & 85.28 & 85.96 & 84.15 & 80.4  & 80.96    & 83.09 & 84.50 & 85.42 & 86.29 \\
STS17                                  & 89.03 & 90.54 & 90.3  & 87.58 & 89.37 & 90.25 & 87.23 & 87.07 & 87.78    & 89.15 & 89.95 & 89.95 & 90.62 \\
STS22                                  & 64.11 & 68.65 & 67.74 & 64.07 & 62.99 & 68.12 & 62.88 & 66.13 & 69.35    & 62.92 & 65.81 & 65.13 & 65.01 \\
STSBenchmark                           & 87.74 & 86.56 & 86.88 & 86.52 & 87.21 & 83.17 & 86.18 & 80.9  & 81.39    & 83.63 & 85.79 & 87.71 & 88.02 \\
\midrule
SummEval & 30.19 & 32.32 & 31.84 & 30.28 & 30.97 & 30.8 & 31.01 & 33.6 & 31.46 & 32.06 & 31.10 & 30.62 & 30.97 \\
\midrule \midrule
Average  & 62.25 & 61.79 & 61.59 & 61.5 & 61.42 & 60.99 & 60.44 & 57.59 & 58.93 & 55.80 & 58.28 & 59.86 & 60.63 \\
\bottomrule[1pt]
\end{tabular}}
\caption{
Deatiled results on MTEB English. We include the scores of top-performing models and the baseline SGPT from the online leaderboard.
%  (retrieved on June 20th, 2023).
}
\label{tab:mteb-en-full}
\end{table*}


==> tables/multicpr_copy.tex <==
\begin{table*}
\centering
\resizebox{2.0\columnwidth}{!}{
\begin{tabular}{@{}c|c|c|c|cc|cc|cc}
\toprule[1pt]
\multicolumn{2}{c|}{\multirow{2}{*}{\bf Model}} &
  {\multirow{2}{*}{\bf Dataset}} &
  {\multirow{2}{*}{\bf Backbone}} &
  \multicolumn{2}{c|}{\bf E-commerce} &
  \multicolumn{2}{c|}{\bf Entertainment video} &
  \multicolumn{2}{c}{\bf Medical} \\ \cmidrule(l){5-10} 
\multicolumn{2}{c|}{} & & &MRR@10 & Recall@1k & MRR@10 & Recall@1k & MRR@10 & Recall@1k \\ \midrule
\multirow{2}{*}{\bf Sparse} & BM25 & - & - & 0.225 & 0.815 & 0.225 & 0.780 & 0.187 & 0.482 \\
 & Doc2Query & - & - & 0.239 & 0.826 & 0.238 & 0.794 & 0.210 & 0.505 \\ \midrule
\multirow{8}{*}{\bf Dense} & 
 % DPR & General & BERT & 0.2106 & 0.7750 & 0.1950 & 0.7710 & 0.2133 & 0.5220 \\
 DPR-1 & In-Domain & BERT & 0.270 & 0.921 & 0.254 & 0.934 & 0.327 & 0.747 \\
 & DPR-2 & In-Domain & BERT-CT & 0.289 & \bf 0.926 & 0.263 & \bf 0.935 & 0.339  & \bf 0.769 \\
\cmidrule{2-10}
& text-embedding-ada-002 & General & GPT & 0.183 & 0.825 & 0.159 & 0.786 & 0.245 & 0.593 \\
& sgpt-bloom-7b1-msmarco & General & BLOOM & 0.242 & 0.840 & 0.227 & 0.829 & 0.311 & 0.675 \\
\cmidrule{2-10}
 & \modelname-bloom-560m & General & BLOOM & 0.156 & 0.802 & 0.149 & 0.749 & 0.245  & 0.571 \\
 & \modelname-bloom-1b1 & General & BLOOM & 0.244 & 0.863 & 0.208 & 0.815 & 0.241  & 0.557 \\
 & \modelname-bloom-3b & General & BLOOM & 0.267 & 0.871 & 0.228 & 0.836 & 0.288  & 0.619 \\
 & \modelname-bloom-7b1 & General & BLOOM & \bf 0.296 & 0.889 & \bf 0.267 & 0.907 & \bf 0.343  & 0.705 \\
 \bottomrule[1pt]
\end{tabular}
}\caption{
Results on Multi-CPR \citep{long2022multicpr}. ``In-Domain'' indicates that the adopted training dataset is from the corresponding domain. ``BERT-CT'' notes that the BERT model is continuing pre-trained with domain corpus.
}\label{tab:multicpr-results}
\end{table*}


==> tables/sts-cross.tex <==
\begin{table*}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccccc|cccccccc}
\toprule
& \multicolumn{7}{c|}{\bf STS-17}   & \multicolumn{8}{c}{\bf STS-22}    \\
\midrule
\bf Model                             & \bf en-ar & \bf es-en & \bf fr-en & \textbf{en}-\textit{de} & \textbf{en}-\textit{tr} & \textit{it}-\textbf{en} & \textit{nl}-\textbf{en} & \textbf{es-en} & \textbf{zh-en} & \textit{de}-\textbf{en} & \textit{de}-\textbf{fr} & \textit{de-pl} & \textbf{es}-\textit{it} & \textbf{fr}-\textit{pl} & \textit{pl}-\textbf{en} \\
\midrule
LASER2                                          & 65.05 & 55.3  & 70.82 & 66.66          & 70.05          & 70.98          & 68.12          & 54.34 & 46.19 & 32.35          & 37.41          & 15.67          & 42.21          & 39.44          & 53.63          \\
LaBSE                                           & 74.51 & 65.71 & 76.98 & 73.85          & 72.07          & 76.99          & 75.22          & 71.86 & 64.02 & 50.14          & 53.28          & \bf 58.69          & 69.69          & 61.98          & 69.41          \\
% all-MiniLM-L12-v2                               & 0.54  & 22.01 & 30.7  & 27.54          & 0.43           & 24.28          & 24.51          & 53.99 & 44.39 & 42.86          & 43.52          & 1.63           & 40.71          & 16.9           & 42.67          \\
% all-MiniLM-L6-v2                                & -4.28 & 16.31 & 37.09 & 35.82          & 4.5            & 24.45          & 29             & 53.42 & 41.64 & 44.04          & 30.07          & 4.93           & 44.27          & 50.71          & 32.8           \\
% allenai-specter                                 & 6.9   & 10.86 & 16.02 & 11.59          & 6.46           & 19.87          & 24.92          & 51.79 & 8.44  & 26.03          & 10.26          & 16.94          & 25.24          & 39.44          & 25.36          \\
% gtr-t5-large                                    & -5.77 & 54.96 & 60.5  & 67.43          & 8.75           & 46.26          & 47.48          & 67.76 & 29.42 & 48.76          & 57.5           & 32.76          & 57.18          & 61.98          & 54.17          \\
% gtr-t5-xl                                       & -3.22 & 60.24 & 62.17 & 70.38          & 17.17          & 59.11          & 56.91          & 69.99 & 28.85 & 53.63          & 55.72          & 27.99          & 60.94          & 61.98          & 60.18          \\
% komninos                                        & 9.08  & -8.18 & 5.81  & -3.11          & -0.45          & 3.64           & 0.44           & 26.97 & 14.05 & 28.65          & 14.77          & 11.21          & 41.1           & 39.44          & 45.55          \\
paraphrase-multilingual-MiniLM-L12-v2           & 81.22 & 84.44 & 76.59 & \bf 84.22          & \bf 76.74          & 82.35          & 81.71          & 67.33 & 65.71 & 52.65          & 51.73          & 44.22          & 47.67          & 50.71          & 69.02          \\
paraphrase-multilingual-mpnet-base-v2           & 80.85 & 86.11 & 81.17 & 83.28          & 74.9           & \bf 84.24          & \bf 82.51          & 70.26 & 67.96 & 50.81          & \bf 62.34          & 40.53          & 53.7           & \bf 84.52          & \bf 73.07          \\
% sentence-t5-base                                & -5.65 & 47.72 & 56.61 & 67.11          & -0.02          & 30.46          & 36.46          & 65.19 & 20.15 & 46.9           & 55.04          & 33.94          & 55.29          & 28.17          & 42.97          \\
% sentence-t5-large                               & -4.71 & 62.62 & 67.86 & 73.62          & -0.42          & 51.86          & 45.95          & 68.09 & 23.1  & 49.93          & 61.58          & 38.83          & 61.58          & 5.63           & 51.72          \\
% sentence-t5-xl                                  & -3.93 & 71.72 & 71.38 & 79.04          & 13.61          & 69.5           & 66.12          & 69.15 & 29    & 49.64          & 62.21          & 34.34          & 65.26          & 50.71          & 58.85          \\
% SGPT-125M-weightedmean-msmarco-specb-bitfit     & 8.21  & 28.78 & 26.34 & 30.18          & 1.04           & 20.73          & 25.05          & 49.51 & 28.68 & 53.07          & 32.97          & 20.45          & 45.78          & 61.98          & 36.8           \\
% SGPT-125M-weightedmean-nli-bitfit               & 1.72  & 21.93 & 18.91 & 25.48          & 2.09           & 16.39          & 23.49          & 32.74 & 26.71 & 53.93          & 25.11          & 20.94          & 35.99          & 5.63           & 20.54          \\
sgpt-bloom-7b1-msmarco                          & 78.07 & 78.22 & 80.46 & 59.1           & 11.8           & 51.58          & 45.85          & 75.06 & 68.45 & 51.16          & 53.28          & 43.05          & 65.5           & 28.17          & 53.31          \\
% paraphrase-multilingual-mpnet-base-v2-KE\_Sieve & 77.6  & 81.59 & 77.16 & 70.4           & 71.04          & 81.52          & 80.7           & 67.29 & 64.45 & 49.09          & 50.6           & 50.44          & 57.93          & 73.25          & 67.72          \\
multilingual-e5-base                            & 71.27 & 76.5  & 80.18 & 82.09          & 63.33          & 80.15          & 79.25          & 73.99 & 69.92 & 54.93          & 59.47          & 39.35          & 66.46          & 73.25          & 70.37         \\
\midrule
\modelname-bloom-560m    & 72.60 & 81.80 & 79.94   & 40.34 & 6.79 & 34.80 & 33.58      & 71.03 & 63.90 &   49.55 & 22.36 & 35.32 & 61.30 & 73.25 & 43.72 \\
\modelname-bloom-1b1  & 79.64 & 85.41 & 83.96 & 52.52 & 4.75 & 45.62 & 46.69 & 73.59 & 65.01 & 51.66 & 39.66 & 26.11 & 67.83 & 84.52 & 60.77   \\
\modelname-bloom-3b   & 79.36 & 85.02 & 86.62 & 64.32 & 12.41 & 61.30 & 53.17 & 73.80 & 68.82 & 53.01 & 53.84 & 39.57 & 70.87 & 39.44 & 57.10 \\
\modelname-bloom-7b1  & \bf 84.41 & \bf 87.67 & \bf 88.31 & 73.84 & 20.07 & 69.42 & 58.20 & \bf 76.54 & \bf 70.88 & \bf 55.17 & 55.02 & 43.88 & \bf 70.13 & 61.98 & 69.34 \\
\bottomrule
\end{tabular}
}
\caption{
Spearman correlation between embedding cosine similarity and labels on STS17 \& 22 cross-lingual testset.
Languages in \textit{italic} are not included in the BLOOM pre-training set.
Reference results are retrieved from MTEB online leaderboard on June 20th, 2023.
}\label{tab:sts-cross}
\end{table*}


==> tables/sts-multi.tex <==
\begin{table*}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cccc|cccccccccc}
\toprule[1pt]
& \multicolumn{4}{c|}{\bf STS-17}              & \multicolumn{10}{c}{\bf STS-22}   \\
\midrule
\bf Model    & \bf ar & \bf en & \bf es & \textit{ko} & \bf ar    & \bf en    & \bf es    & \bf fr    & \bf zh    & \textit{de} & \textit{it} & \textit{pl} & \textit{ru} & \textit{tr} \\
\midrule
LASER2                                          & 67.47 & 76.73 & 79.67 & 70.52          & 42.57 & 39.76 & 54.92 & 58.61 & 49.41 & 25.69       & 60.31       & 18.34       & 39.24       & 36.97       \\
LaBSE                                           & 69.07 & 79.45 & 80.83 & 71.32          & 57.67 & 60.97 & 63.18 & 77.95 & 63.02 & 48.58       & 72.22       & \bf 39.3        & 57.49       & 58.15       \\
% all-MiniLM-L12-v2                               & 58.71 & 88.63 & 78.37 & 43.37          & 17.54 & 65.67 & 43.98 & 69.51 & 33.15 & 22.53       & 47.48       & 19.22       & 11.19       & 21.6        \\
% all-MiniLM-L6-v2                                & 50.89 & 87.59 & 76.12 & 43.39          & 22.64 & 67.21 & 54.78 & 77    & 44.93 & 31.04       & 60.4        & 26.77       & 14.72       & 33.69       \\
% allenai-specter                                 & 27.14 & 69.63 & 55.45 & 8.08           & 19.57 & 55.06 & 48.89 & 53.92 & 16.35 & 17.31       & 39.43       & 13.56       & 1.11        & 31.73       \\
% gtr-t5-large                                    & 10.19 & 83.93 & 82.74 & 8.96           & 34.97 & 64.3  & 57.49 & 78.7  & 27.32 & 51.7        & 67.67       & 30.68       & 15.36       & 58.12       \\
% gtr-t5-xl                                       & 9.06  & 84.9  & 81.93 & 8.9            & 37.66 & 66.61 & 59.14 & 79.43 & 31.16 & 50.58       & 67.14       & 33.74       & 32.69       & 55.79       \\
% komninos                                        & 13.78 & 76.91 & 48.23 & 2.54           & 32.42 & 53.89 & 48.53 & 49.43 & 4.78  & 33.04       & 57.77       & 12.47       & 19.44       & 47.38       \\
paraphrase-multilingual-MiniLM-L12-v2           & 79.16 & 86.87 & 85.56 & 77.03          & 46.2  & 61.72 & 56.56 & 70.55 & 58.75 & 44.64       & 55.22       & 33.74       & 57.08       & 53.39       \\
paraphrase-multilingual-mpnet-base-v2           & 79.1  & 86.99 & 85.14 & \bf 83.41          & 52.19 & 63.06 & 59.91 & 74.3  & 61.75 & 46.7        & 60.65       & 33.65       & 58.74       & 56.3        \\
% sentence-t5-base                                & 13.36 & 89.57 & 79.94 & 10.06          & 31.2  & 62.66 & 53.81 & 77.69 & 32.9  & 42.08       & 60.65       & 24.42       & 12.13       & 40.45       \\
% sentence-t5-large                               & 10.75 & 88.99 & 82.74 & 9.44           & 27.01 & 62.39 & 57.68 & 75.01 & 30.47 & 43.73       & 62.01       & 25          & 14.21       & 47.3        \\
% sentence-t5-xl                                  & 11.13 & 88.91 & 83.42 & 9.61           & 29.6  & 64.32 & 58.16 & 77.49 & 33.55 & 47.72       & 66.91       & 27.04       & 26.63       & 43.36       \\
% SGPT-125M-weightedmean-msmarco-specb-bitfit     & 55.62 & 84.95 & 71.88 & 52.39          & 28.19 & 65.66 & 49.81 & 67.66 & 25.49 & 21.99       & 48.25       & 23.31       & 9.07        & 34.66       \\
% SGPT-125M-weightedmean-nli-bitfit               & 54.16 & 87.33 & 67.8  & 45.66          & 5.17  & 59.64 & 43.05 & 54.56 & 6.52  & 11          & 33.68       & 14.91       & 3.36        & 3.82        \\
sgpt-bloom-7b1-msmarco                          & 76.42 & 87.07 & 86    & 66.89          & \bf 58.67 & \bf 66.13 & 65.41 & \bf 80.38 & \bf 66.78 & 30.05       & 65.65       & 31.13       & 43.36       & 47.14       \\
% paraphrase-multilingual-mpnet-base-v2-KE\_Sieve & 76.04 & 85.4  & 82.77 & 77             & 52.61 & 58.63 & 57.23 & 72.79 & 60    & 41.84       & 64.17       & 36.37       & 53.35       & 52.71       \\
multilingual-e5-base                            & 74.52 & 87.83 & 86.74 & 79.95          & 57.87 & 61.83 & \bf 66.58 & 74.8  & 65.63 & \bf 55.95       & \bf 77.76       & 34.13       & \bf 60.66       & \bf 63.7       \\
\midrule
% \modelname-bloom-560m      &   80.60 & 89.15 & 85.65 & 57.28    & 54.82 & 62.92 & 56.31 & 78.73 & 40.97 & 26.63 & 62.61 & 15.06 & 28.77 & 22.10 \\
% \modelname-bloom-1b1    & 81.13 & 89.95 & 87.33 & 61.89 & 55.00 & 65.81 & 59.79 & 81.25 & 54.08 & 37.51 & 68.87 & 27.98 & 43.14 & 42.33 \\
% \modelname-bloom-3b    & 82.06 & 89.95 & 86.74 & 63.22  & 55.60 & 65.13 & 61.02 & 81.55 & 57.36 & 42.25 & 72.51 & 29.71 & 48.75 & 53.09 \\
% \modelname-bloom-7b1   & \bf 83.75 & \bf 90.62 & \bf 88.32 & 64.81 & 56.32 & 65.01 & 62.07 & \bf 82.99 & 60.26 & 43.92 & 71.32 & 31.26 & 49.39 & 54.59 \\
en-all-bloom-1b1   & 81.31 & 89.85 & 86.36 & 61.43   & 52.64 & 61.93 & 54.44 & 75.19 & 55.86 & 23.93 & 70.14 & 32.71 & 44.47 & 42.51 \\
en-all-bloom-3b    & 81.67 & 90.77 & 86.60 & 66.12   & 48.62 & 59.82 & 54.71 & 70.57 & 54.39 & 22.16 & 73.32 & 33.62 & 46.61 & 43.20 \\
en-all-bloom-7b1   & \bf 83.41 & \bf 91.60 & \bf 87.72 & 66.53   & 49.99 & 60.80 & 59.94 & 76.77 & 57.47 & 31.98 & 73.06 & 32.96 & 48.74 & 51.10 \\
\bottomrule[1pt]
\end{tabular}
}\caption{
Spearman correlation between embedding cosine similarity and labels on STS17 \& 22 multilingual testset.
Language codes in \textit{italic} are not included in the BLOOM pre-training.
Reference results are retrieved from MTEB. % online leaderboard on June 20th, 2023.
}\label{tab:sts-multi}
\end{table*}


==> tables/tatoeba.tex <==
\begin{table*}
\resizebox{\textwidth}{!}{
\begin{tabular}{lc|cccccccccccccccc}
\toprule[1pt]
Model                                 & Avg.   & ben-en & cat-en & eus-en & fra-en & hin-en & ind-en & mal-en & mar-en & por-en & spa-en & swh-en & tam-en & tel-en & urd-en & vie-en & xho-en \\
\midrule
LaBSE                                 & \bf 93.83 & \bf 88.55  & 95.38  & \bf 95.01  & \bf 94.86  & 96.87  & \bf 93.66  & \bf 98.45  & 92.65  & 94.14  & \bf 98.4   & \bf 84.5   & \bf 89     & \bf 97.86  & 93.22  & 97.2   & \bf 91.55  \\
paraphrase-multilingual-MiniLM-L12-v2 & 63.63 & 36.48  & 94.42  & 23.18  & 91.72  & 97.62  & 92.74  & 32.2   & 92.38  & 92.13  & 95.42  & 14.48  & 24.64  & 36.4   & 94.57  & 95.12  & 4.52   \\
paraphrase-multilingual-mpnet-base-v2 & 76.07 & 64.9   & \bf 96.05  & 31.33  & 93.12  & \bf 97.75  & 93.5   & 88.46  & \bf 93.83  & 93.02  & 97     & 16.02  & 73.6   & 79.73  & \bf 95.12  & \bf 97.23  & 6.53   \\
sgpt-bloom-7b1-msmarco                & 70.14 & 75.98  & 88.31  & 53.38  & 91.44  & 85.23  & 88.04  & 83.3   & 45.53  & 92.62  & 94.48  & 16.74  & 72.76  & 64.62  & 70.1   & 94.2   & 5.51   \\
multilingual-e5-base                  & 85.31 & 81.05  & 84.09  & 56.16  & 92.76  & 93     & 90.26  & 96.72  & 86.62  & 92.74  & 96.97  & 66.81  & 85.12  & 88.49  & 86.2   & 94.68  & 73.24  \\
\midrule
\modelname-bloom-560m                                  & 64.79 & 70.14  & 81.55  & 42.35  & 91.65  & 85.35  & 85.46  & 73.36  & 47.23  & 92.08  & 95.48  & 14.52  & 62.26  & 35.84  & 61.62  & 92.86  & 4.83   \\
\modelname-bloom-1b1                                   & 72.30 & 78.76  & 84.54  & 59.64  & 92.77  & 91.53  & 88.30  & 85.56  & 52.67  & 92.52  & 96.05  & 16.31  & 77.30  & 69.05  & 68.96  & 94.57  & 8.30   \\
\modelname-bloom-3b                                    & 77.02 & 80.65  & 91.17  & 63.81  & 93.53  & 92.87  & 90.54  & 93.12  & 65.18  & 93.62  & 97.77  & 25.43  & 84.66  & 79.30  & 76.77  & 96.05  & 7.79   \\
\modelname-bloom-7b1                                   & 79.12 & 83.89  & 90.24  & 74.53  & 94.32  & 94.88  & 91.91  & 95.05  & 71.56  & \bf 94.43  & 98.13  & 27.81  & 81.87  & 80.56  & 82.87  & 95.83  & 7.96  \\
\bottomrule[1pt]
\end{tabular}}
\caption{Tatoeba test (15 langs included by the BLOOM pre-training). Reference results are retrieved from MTEB online leaderboard on June 20th, 2023.}
\label{tab:tatoeba}
\end{table*}

